ROLL: Visual Self-Supervised Reinforcement Learning with Object Reasoning

Current image-based reinforcement learning (RL) algorithms typically operate on the whole image without performing object-level reasoning. This leads to inefficient goal sampling and ineffective reward functions. In this paper, we improve upon previous visual self-supervised RL by incorporating object-level reasoning and occlusion reasoning. Specifically, we use unknown object segmentation to ignore distractors in the scene for better reward computation and goal generation; we further enable occlusion reasoning by employing a novel auxiliary loss and training scheme. We demonstrate that our proposed algorithm, ROLL (Reinforcement learning with Object Level Learning), learns dramatically faster and achieves better final performance compared with previous methods in several simulated visual control tasks. Project video and code are available at https://sites.google.com/andrew.cmu.edu/roll.

==> inputs/draft.tex <==
\section{Core Idea of the paper}
   Self-supervised RL usually assumes no prior information about the task. However, we should try to inject prior knowledge about the task when such knowledge can be easily obtained. 
    For image-based RL tasks, segmented images can be obtained for free without human annotations if the background is static. In this paper, 
    
\begin{itemize}
    \item We train an image segmentation module to focus on the task-relevant part of the observation, and extract a more effective reward function for self-supervised learning.
    
    \item We carefully design the architecture of the reward extractor, and add a novel auxiliary loss to make it robust to object occlusions.
    
    \item We show our method helps to dramatically reduces the sample complexity compared with baselines, in several simulated visual control tasks, and a real-World vision-based robotic manipulation task.
    
    
    

    \item Segmentation is cheap, and we use segmentation to provide a more meaningful reward signal for RL learning.
    
    More explanations of the method:
    In settings where the RL agent has only high-dimensional image observations and no access to ground-truth rewards, previous methods use a VAE to encode the images into a latent space, and then use the L2 distance between the latent vector of the current observation and the latent vector of the goal image as reward. Using a reconstruction loss, the VAE learns to encode everything in the image, e.g., the background, the objects, and the robot. However, for object manipulation tasks, we ultimately only care about the object that is being manipulated. Therefore, the reward function derived from a latent space that encodes everything in the image is less clean and less effective due to its redundant and even distracting information. Segmented images that contain only the manipulated objects can be obtained for free without human annotations if the background is static. We propose to use light-weight segmentation methods to remove the distracting elements in the image (e.g., the background, the robot), keep only the objects,  and learn a latent space using the segmented images, providing a cleaner and better reward function for RL learning to achieve better performances.
    

\end{itemize}
